On the Relation between Sensitivity and Accuracy in In-context Learning

In-context learning (ICL) suffers from oversensitivity to the prompt, making it unreliable in real-world scenarios. We study the sensitivity of ICL with respect to multiple perturbation types. First, we find that label bias obscures the true sensitivity, and therefore prior work may have significantly underestimated ICL sensitivity. Second, we observe a strong negative correlation between ICL sensitivity and accuracy: predictions sensitive to perturbations are less likely to be correct. Motivated by these findings, we propose \textsc{SenSel}, a few-shot selective prediction method that abstains from sensitive predictions. Experiments on ten classification datasets show that \textsc{SenSel} consistently outperforms two commonly used confidence-based and entropy-based baselines on abstention decisions.

==> archived/Introduction.tex <==
% \chen{Could we split this giant latex file into multiple files, where each section is a file?}

% \chen{In general, i think the intro is ok, but we need more insights from experiments to make it stronger.}
% \yanda{I've added to the intro and the paper body the takeawys from the MC tasks. Let me know if there's anything else you think we could add.}

% \hh{Please make sure that all figures are directly output to  pdf format so that it's not blurred when zoomed in.}
% \yanda{Fixed.}

\section{Introduction}

\hh{High level comment on intro structure:
1. Move first paragraph and directly motivate the few-shot selective classification method.
2. Challenges in FSSC: 1) not enough examples for tuning the predictor; 2) LM prediction is poorly calibrated so cannot directly be used as confidence.
3. Motivate our method based on the observation that high sensitivity correlates with likelihood of mistakes.
4. Results.
}

\hh{Also, it might be helpful to have an illustration of the method (i.e. a figure 1) if we have space.}

\begin{figure*}[t]
\centering
\includegraphics[scale=0.38]{correlation.pdf}
\caption{\label{fig:sensitivity-correlation}We plot LM sensitivity against prediction accuracy on all test examples on five classification benchmarks for each of the three perturbation sets (Section~\ref{sec:perturbation-sets}). We observe a strong negative correlation between LM sensitivity and prediction accuracy across all 10 tasks and all three perturbation sets. Prototypical calibration is applied to address label bias.}
\end{figure*}

% \hh{Terminology:
% Few-shot ICL: doesn't ICL imply few-shot?
% Selective prediction with abstention: selective prediction and abstention are redundant.
% }
% \yanda{Thanks for pointing this out. I've fixed this for the entire paper.}

Few-shot learning (FSL) refers to a model's ability to quickly learn a new task based on few labeled examples. Recently, prompting language models (LMs) for FSL has achieved remarkable progress via in-context learning (ICL) \cite{brown2020language}. 
%Because minimal data annotation efforts are needed to learn a new task, ICL systems have huge potential to be deployed to \textit{the real world} to tackle various tasks such as clinical healthcare delivery \cite{Korngiebel2021ConsideringTP, Sezgin2022OperationalizingAI}, legal consulting \cite{eliot2021generative}, and user intent modeling \cite{hu2022context}.
% \chen{Could you add an example of which systems are deployed into real world? If not, we need to rephrase it.}
Despite its remarkable progress, ICL
% \chen{Are there references for these issues? I suggest only mentioning sensitivity, as the second is the outcome of sensitivity issue.}
is known to be fragile as its predictions are over-sensitive to the prompt, such as the wording of the task instruction \cite{schick-schutze-2021-exploiting, jiang-etal-2020-know, gao-etal-2021-making} and the ordering of the few-shot examples \cite{zhao2021calibrate, liu2021makes}.
% \chen{TODO: have a figure showing sensitivity, and sensitivity is negatively related to accuracy.}
% \yanda{Done.}

\hh{The second para does not directly follow from the first. If the problem is that ICL is over-sensitive to prompts, isn't the most logical next step to reduce sensitivity to prompts? Abstention is justifiable even without the sensitivity issue, so mixing the two is a bit confusing.}

In this paper, we systematically study ICL sensitivity with respect to different types of perturbations: automatic instruction perturbations, human-written instruction perturbations, and in-context example ordering perturbations. Our main observations are two-fold.

First, we observe that previous work may have significantly underestimated ICL sensitivity due to label bias.

% \chen{I think we should reorder these sentences. 1) It's important to have abstention mechanism in real world as we do not want to give wrong predictions 2) Define abstention and what tradtional methods do  3) in ICL scenarios, it's a challenging problem, because it is sensitive}
When ICL systems are deployed to the real-world, it is important to have an abstention mechanism to avoid giving wrong predictions, especially in high-stakes domains such as medical \cite{Korngiebel2021ConsideringTP, Sezgin2022OperationalizingAI} and legal \cite{eliot2021generative}. In this work, 
% we propose the task\hh{We should probably not claim that we formulated a new task since selective classification is well studied. Perhaps rephrase to "our goal is ...".} of
we focus on \textit{selective prediction} in the \textit{few-shot} setting,
% \textit{selective few-shot prediction with abstention}, 
where ICL systems are asked to abstain on examples that they are not confident about how to predict, so as to improve the average accuracy on the predicted examples at the cost of lowering the prediction coverage (Section~\ref{sec:selective-prediction-fsl}).
% \chen{fairness is not a domain}
% \chen{I suggest combining this paragraph with the previous one, and largely shorted it.}
% \chen{The previous two sentences can be shortened or combined.}
% Selective prediction also enables better human-LM collaboration as humans can step in to handle examples that LMs abstain on.
% The key of selective prediction is to estimate the confidence of LM's prediction on each example. During test time, LMs abstain on examples where LM predictions are estimated to be not confident.

\hh{We should have a brief paragraph here on the *challenges* of few-shot selective classification. Why can't we just apply existing selective classification methods? Then the next paragraph would be about how our method addresses the challenges.}


%\hh{The first sentence is a bit disconnected from the rest. This paragraph is mainly about the observation of the sensitivity-accuracy relationship.}
%\yanda{I moved the first sentence to the next paragraph. We need a transition sentence here. @CZ could you take a look at this?}
\hh{Right now we are saying that we have a hypothesis based on our intuition and we verified it through experiments. But this hypothesis is neither intuitive nor grounded in some theory. It's better to just say that our approach builds upon a key *observation* that ...}
Our key intuition is that LM sensitivity is negatively correlated with prediction accuracy -
% \chen{This contradicts sensitivity is related to accuracy.}
\chen{Say something like that: to successfully abstain examples, we need to identify examples that are likely to have low prediction accuracy. Then we can say accuracy is negatively correlated to sensitivity. }
\hh{Some of the first paragraph content on sensitivity can go here.}
if a LM prediction is very sensitive to various perturbations of the prompt format\hh{Say prompt? The perturbations are not just on "format".} (e.g., the instruction wording and the few-shot example ordering), then this prediction is unlikely to be correct\hh{Why is it the case? We can't just push the result to the reader. A potential explanation is that Min et al and Xie et al suggest that prompt is mainly used to elicit task-specific knowledge acquired during pretraining by the LLM; if the model is sensitive to the elicitation content (i.e. the prompt), then it suggests that the LM did not learn the task well during pretraining, thus likely to make mistakes. If we don't have a good reason, we can also just say we observed empirically that...}.
We validate our hypothesis through a sensitivity study, where we discover a strong negative correlation between LM ICL sensitivity and prediction accuracy on 10 classification benchmarks (Section~\ref{sec:sensitivity-study}, Figure~\ref{fig:sensitivity-correlation}). % encompassing emotion classification, topic classification, ontology classification and question-answer verification.
% \chen{Can we claim only from classification tasks (I guess reviewers might have similar concerns)}
% The correlation is even stronger when decision boundary adjustment methods are applied to address label bias issues. \chen{Without context, it's hard to understand this sentence.}
% \chen{Need a better transition sentence, something like based on study, we think sensitivity is a better signal for abstention}

Motivated by the sensitivity study, we conjecture that LM sensitivity is a better\hh{-> useful. Better than what?} signal for abstention. We propose few-shot selective prediction via LM sensitivity, where the LM abstains on examples where predictions are most sensitive to prompt perturbations
% Unlike
% \chen{different from -> unlike}
% previous selective prediction methods that rely on the confidence estimated by the LM itself,
% \hh{Selective prediction doesn't have to use confidence estimated by LM itself. Also if the LM is calibrated, it would be optimal to use the output probabilities. I think we can directly say motivated by the observation, we use sensitivity to abstain. Then say that the experiments show that it's better than using model confidence.}
% we use LM sensitivity with respect to prompt perturbations to estimate the confidence of a LM prediction 
(Section~\ref{sec:sensitivity-selective-prediction-method}).
% We benchmark our sensitivity-based selective prediction method on 10 classification benchmarks encompassing emotion classification, topic classification, ontology classification and question-answer verification. 
% \chen{In the previous paragraph, we already do experiments on these datasets}
Experiment results show that our sensitivity-based selective prediction method\hh{Give it a name?} \chen{maybe \textsc{SenSel}}\hh{Then maybe the full name should be sensitivity-based selective prediction?} consistently outperforms a confidence-based selective prediction 
%the MaxProb
%\hh{The readers don't know MaxProb yet.}
baseline.
\hh{``Confidence'' is a concept that needs to be defined. Can we just say baselines or methods using model probabilities?}

We further analyze the results to understand on which tasks our sensitivity-based selective prediction method works. We discover a negative correlation between the LM sensitivity on a task and the effectiveness of our sensitivity-based abstention method on that task (Figure~\ref{fig:sensitivity-performance}). Our sensitivity-based selective prediction method is most effective on tasks where the LM predictions are over-sensitive, which we claim are also the tasks where an effective abstention mechanism is most crucial.
% Analysis further shows that our sensitivity-based selective prediction method is most effective on tasks where the LM is highly fragile\hh{What does this mean?} and over-sensitive, which we claim is also the setting where an effective abstention mechanism is most crucial. 
On the other hand, because our selective prediction method relies on LM sensitivity, it does not work well on tasks where the LM predictions are stable and not over-sensitive \hh{What are the properties of these tasks? It reads a bit like it works when it works and falls short of a deeper reason.}.
\yanda{Do you think the new paragraph is clearer?}
\textcolor{red}{[TODO: Read results and come back to this.]}
% \chen{We should probably talk about take-aways from non-classification task}
% \yanda{I agree that we should talk about the take-aways from non-classificaion tasks, i.e., our approach works the best when LM is sensitive and does not work when LM is not sensitive. The question is whether we should present that takeaway through classification tasks or MC tasks. If it's through MC tasks then we need to present additional datasets and numbers. I have added a paragraph in Section 4 results that introduces this takeaway based on the classification tasks. Do you think this is good enough or we need to include the MC tasks?}
% \chen{I think reviewers will ask tasks other than classification, it is better to address it beforehand.}


==> archived/Related_Work.tex <==
\section{Related Work}
\hh{
The in-context learning section should be mainly about selective prediction or calibration whereas right now it's mostly about reducing sensitivity.
I suggest we restructure it as follows:
1. selective classification;
2. model calibration;
3. their applications in in-context learning or LLMs.
1 and 2 talk about general techniques and 3 talks about related work in in-context learning.
In addition, we should be clear about the connection between 1 and 2. 1 aims to trade-off accuracy and coverage. 2 aims to produce prediction probabilities that correspond to likelihood of a correct prediction,
although a calibrated output from 2 can be used for 1.
Actually another piece of related work in ICL is decision boundary correction and we should include it; these are all related goals and we should articulate the difference and connections.
}

\paragraph{In-context Learning}
Recently, prompting LMs for few-shot learning has achieved remarkable success via in-context learning \cite{brown2020language}. Despite its empirical success, in-context learning is known to suffer from over-sensitivity to instruction wording \cite{schick-schutze-2021-exploiting, jiang-etal-2020-know, gao-etal-2021-making}\hh{Sameer has a recent work that shows ICL performance is related to term frequency in pretraining, which might be relevant.} and example ordering \cite{zhao2021calibrate, liu2021makes}. Several methods have been proposed to reduce LM sensitivity. \citet{zhou2022prompt} propose to explicitly fine-tune the LM to output consistent predictions across diverse prompts, so as to achieve better zero-shot accuracy and reduce sensitivity. \citet{chen-etal-2022-meta} propose to meta-train LMs to learn in-context learning, and show that meta-learning effectively reduces LM sensitivity with respect to example ordering and example selection. Despite these efforts, state-of-the-art instruction-tuned LMs such as T0\hh{Is this still sota? I thought InstructGPT is better.} \cite{sanh2021multitask} are still highly sensitive to the prompt format.

\hh{Selective prediction is independent of using LMs. We should describe it in the context of general ML models.}
\paragraph{Selective Prediction}
In selective prediction, LMs\hh{Doesn't have to be LM.} are asked\hh{Awkward. The goal of selective prediction is to ...} to abstain on examples that they are not confident about, so as to avoid giving wrong predictions \cite{5222035, foundations2010}. MaxProb estimates the confidence of a LM prediction as the probability the LM assigns to that prediction, and is shown to be a simple yet effective selective prediction method \cite{hendrycks2017a, lakshminarayanan2017simple, xin-etal-2021-art}. Unfortunately, because ICL predictions are over-sensitive to various artifacts \cite{schick-schutze-2021-exploiting, jiang-etal-2020-know, zhao2021calibrate}, selective prediction based on MaxProb is also over-sensitive and fragile.

Previous work has also proposed to train a separate calibrator to estimate prediction confidence \cite{platt,geifman2017selective, geifman2019selectivenet, kamath-etal-2020-selective}, but training such a calibrator requires large amount of task-specific labeled data which is not available under the few-shot setting, which we target in our work. 

\hh{Can we have a separate section (including the content below) on calibration?}
Our work is most similar to predictive uncertainty estimation with Bayesian inference, which is approximated by evaluating prediction sensitivity with respect to model weight perturbations such as parameter dropout \cite{dong-etal-2018-confidence, 10.5555/3045390.3045502} or random noise injection \cite{dong-etal-2018-confidence}. Different from previous work, we use the sensitivity with respect to the input prompt format as the signal to abstain.

==> archived/Related_Workv2.tex <==
\section{Background}
%We first introduce relevant concepts related to ICL over LMs, and then 
%describe existing approaches for selective prediction and model calibration.

% \hh{High level comment: I think we should put ICL and label bias in section 3 and the rest in section 4 (see comments below too). There is a lot of background knowledge here and the reader may get lost without knowing why these are needed.}


==> archived/tab_auc_exord.tex <==
\begin{table*}[t]
\fontsize{9.5}{9.5}\selectfont
% \small
\setlength{\tabcolsep}{3pt}
\centering
\begin{tabular}{llccccccccccc}
\toprule
Adj. & Method & AG News & ARP & DBP & Emo & CARER & WikiQA & YAT & LYR & YRFS & MR & Avg \\
\cmidrule{2-13}
% \multirow{3}{*}{None} & F1@Cov100 & 44.6 & 65.6 & 44.8 & 26.0 & 14.1 & 48.7 & 9.7 & 87.6 & 34.4 & 57.8 & 43.3 \\
% \cmidrule{2-13}
% & \textsc{MaxProb} & 41.4 & 72.5 & 52.1 & 28.8 & 15.3 & 49.7 & 10.5 & 93.5 & 32.5 & 64.5 & 46.1 \\
% \cmidrule{2-13}
% & \textsc{SenSel}-ExOrd & 44.6 & 69.7 & 43.0 & 30.6 & 12.6 & 49.2 & 9.7 & 96.9 & 35.1 & 60.6 & 45.2 \\
% \midrule
\multirow{3}{*}{CC} & F1@Cov100 & 54.2 & 94.2 & 78.0 & 29.3 & 29.0 & 50.8 & 29.2 & 90.5 & 38.9 & 70.9 & 56.5 \\
\cmidrule{2-13}
& \textsc{MaxProb} & 52.5 & \textbf{98.5} & 87.8 & 34.0 & 32.6 & 50.5 & 31.0 & 96.2 & 37.1 & 74.9 & 59.5 \\
\cmidrule{2-13}
& \textsc{SenSel}-ExOrd & 54.0 & 97.7 & 85.1 & \textbf{35.5} & \textbf{33.4} & \textbf{51.1} & \textbf{34.6} & \textbf{97.3} & \textbf{40.3} & 76.8 & 60.6 \\
\midrule
\multirow{3}{*}{PC} & F1@Cov100 & 64.5 & 94.5 & 73.3 & 20.8 & 25.3 & 41.9 & 23.8 & 90.7 & 39.6 & 84.3 & 55.9 \\
\cmidrule{2-13}
& \textsc{MaxProb} & 66.5 & 97.5 & 76.7 & 25.3 & 27.7 & 43.5 & 27.4 & 94.4 & 38.5 & 91.9 & 58.9 \\
\cmidrule{2-13}
& \textsc{SenSel}-ExOrd & \textbf{66.6} & 97.7 & \textbf{91.9} & 25.9 & 31.5 & 44.2 & 30.9 & \textbf{97.3} & \textbf{40.3} & \textbf{92.4} & \textbf{61.9} \\
\bottomrule
\end{tabular}
\caption{\label{tab:auc_exord} We compare our sensitivity-based selective prediction method based on example ordering perturbations to the \textsc{MaxProb} baseline. F1@Cov100: F1 scores when no abstention is applied. All scores except F1@Cov100 are AUC scores under the F1-coverage curves (Section~\ref{sec:selective-eval}). Our sensitivity-based \textsc{SenSel}-ExOrd method consistently outperforms \textsc{MaxProb} when decision boundary adjustment methods are applied.}
\end{table*}

==> archived/tab_auc_inst.tex <==
\begin{table*}[t]
\fontsize{9.5}{9.5}\selectfont
% \small
\setlength{\tabcolsep}{3pt}
\centering
\begin{tabular}{llccccccccccc}
\toprule
Adj. & Method & AG News & ARP & DBP & Emo & CARER & WikiQA & YAT & LYR & YRFS & MR & Avg \\
\cmidrule{2-13}
% \multirow{4}{*}{None} & F1@Cov100 & 51.9 & 80.9 & 22.9 & 19.2 & 21.9 & 49.0 & 39.3 & 88.0 & 44.3 & 55.6 & 47.3 \\
% \cmidrule{2-13}
% & \textsc{MaxProb} & 54.7 & 82.4 & 31.3 & 21.7 & 29.1 & \textbf{50.1} & 47.5 & 95.7 & 40.9 & 60.7 & 51.4 \\
% \cmidrule{2-13}
% & \textsc{SenSel}-Inst-H & 61.9 & 81.5 & 24.3 & 21.7 & 21.3 & 49.2 & 37.7 & 90.8 & 40.9 & 54.3 & 48.4 \\
% \cmidrule{2-13}
% & \textsc{SenSel}-Inst-A & 56.6 & 82.3 & 25.7 & 20.5 & 21.4 & 49.2 & 44.6 & 90.1 & 39.2 & 54.0 & 48.4 \\
% \midrule
\multirow{4}{*}{CC} & F1@Cov100 & 55.5 & 85.8 & 47.6 & 15.5 & 31.6 & 34.7 & 42.5 & 86.3 & 50.3 & 79.8 & 53.0 \\
\cmidrule{2-13}
& \textsc{MaxProb} & 57.7 & 87.7 & 52.3 & 21.2 & 40.0 & 35.4 & 45.2 & 95.4 & 50.5 & 86.9 & 57.2 \\
\cmidrule{2-13}
& \textsc{SenSel}-Inst-H & 65.9 & 93.2 & 62.2 & 21.4 & \textbf{40.8} & 41.9 & 49.5 & 94.1 & \textbf{56.4} & 83.0 & 60.8 \\
\cmidrule{2-13}
& \textsc{SenSel}-Inst-A & 57.0 & 86.8 & 53.9 & 18.3 & 37.3 & 39.6 & \textbf{49.6} & 90.8 & 54.1 & 89.7 & 57.7 \\
\midrule
\multirow{4}{*}{PC} & F1@Cov100 & 65.7 & 91.6 & 47.9 & 25.2 & 28.6 & 36.0 & 38.5 & 87.1 & 44.4 & 84.0 & 54.9 \\
\cmidrule{2-13}
& \textsc{MaxProb} & 65.4 & 94.6 & 50.6 & 27.4 & 33.3 & 38.0 & 43.5 & 91.3 & 43.2 & 92.0 & 57.9 \\
\cmidrule{2-13}
& \textsc{SenSel}-Inst-H & \textbf{70.3} & \textbf{96.8} & \textbf{69.0} & \textbf{33.0} & 39.1 & 38.7 & 46.1 & \textbf{96.5} & 46.9 & \textbf{94.1} & \textbf{63.1} \\
\cmidrule{2-13}
& \textsc{SenSel}-Inst-A & 64.9 & 94.7 & 65.4 & 30.8 & 37.1 & 40.6 & 47.1 & 95.7 & 44.0 & 90.4 & 61.1\\
\bottomrule
\end{tabular}
\caption{\label{tab:auc_inst} We compare our sensitivity-based selective prediction method based on instruction perturbations to the \textsc{MaxProb} baseline. F1@Cov100: F1 scores when no abstention is applied. All scores except F1@Cov100 are AUC scores under the F1-coverage curves (Section~\ref{sec:selective-eval}). Our sensitivity-based \textsc{SenSel}-Inst method consistently outperforms the \textsc{MaxProb} baseline when decision boundary adjustment methods are applied.}
\end{table*}

==> archived/tab_label_bias.tex <==
\begin{table*}[t]
\centering
\fontsize{9.8}{10}\selectfont
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lccccccccccc}
\toprule
& AG News & ARP & DBP & Emo & CARER & WikiQA & YAT & LYR & YRFS & MR & Avg \\
\cmidrule(lr){2-12}
Ground-truth & 26.5 & 50.1 & 8.0 & \textbf{85.4} & 35.2 & 95.0 & 11.7 & 50.5 & 21.0 & 50.0 & 43.3 \\
\cmidrule(lr){1-12}
Prediction & \textbf{65.4} & \textbf{75.2} & \textbf{47.9} & 78.9 & \textbf{86.1} & \textbf{100.0} & \textbf{73.5} & \textbf{59.0} & \textbf{51.7} & \textbf{85.3} & \textbf{72.3} \\
\bottomrule
\end{tabular}
\caption{\label{tab:label-bias} The percentage of the majority \textit{predicted} label among all examples is consistently higher than the percentage of the majority \textit{ground-truth} label among all examples, which indicates that LMs suffer from label bias.}
\end{table*}

==> archived/tab_sensitivity.tex <==
\begin{table*}[t]
% \fontsize{9.5}{9.5}\selectfont
\small
\setlength{\tabcolsep}{3pt}
\centering
\begin{tabular}{llccccccccccc}
\toprule
Adjustment & Perturb Set & AGNews & ARP & DBP & Emo & CARER & WikiQA & YAT & LYR & YRFS & MR & Avg \\
\cmidrule{2-13}
\multirow{3}{*}{None} & Inst - H & \textbf{0.415} & \textbf{0.194} & 0.389 & 0.460 & 0.405 & 0.011 & 0.541 & 0.203 & 0.307 & 0.191 & 0.312 \\
\cmidrule{2-13}
& Inst - A & 0.132 & 0.050 & 0.144 & 0.199 & 0.239 & 0.006 & 0.180 & 0.071 & 0.217 & 0.060 & 0.130 \\
\cmidrule{2-13}
& Ex. Ord. & 0.197 & 0.117 & 0.169 & 0.326 & 0.124 & 0.000 & 0.359 & 0.122 & 0.293 & 0.134 & 0.184 \\
\midrule
\multirow{3}{*}{CC} & Inst - H & 0.407 & 0.164 & 0.435 & 0.571 & 0.439 & \textbf{0.518} & 0.517 & 0.187 & 0.347 & \textbf{0.199} & 0.378 \\
\cmidrule{2-13}
& Inst - A & 0.123 & 0.070 & 0.168 & 0.270 & 0.303 & 0.201 & 0.145 & 0.058 & 0.231 & 0.125 & 0.170 \\
\cmidrule{2-13}
& Ex. Ord. & 0.121 & 0.034 & 0.105 & 0.387 & 0.291 & 0.050 & 0.350 & 0.084 & 0.302 & 0.191 & 0.191 \\
\midrule
\multirow{3}{*}{PC} & Inst - H & 0.322 & 0.093 & \textbf{0.619} & \textbf{0.645} & \textbf{0.691} & 0.445 & \textbf{0.694} & \textbf{0.209} & 0.445 & 0.135 & \textbf{0.430} \\
\cmidrule{2-13}
& Inst - A & 0.245 & 0.046 & 0.539 & 0.543 & 0.634 & 0.198 & 0.569 & 0.071 & 0.396 & 0.085 & 0.333 \\
\cmidrule{2-13}
& Ex. Ord. & 0.205 & 0.028 & 0.318 & 0.514 & 0.613 & 0.156 & 0.681 & 0.064 & \textbf{0.456} & 0.119 & 0.315 \\
\bottomrule
\end{tabular}
\caption{\label{tab:sensitivity}ICL sensitivity with respect to different perturbation sets under different decision boundary adjustment methods. We observe that ICL is consistently sensitive with respect to all three perturbation sets, especially when decision boundary adjustment methods are applied to mitigate label bias. 
%Inst - H: Perturb Instruction - Human. Inst - A: Perturb Instruction - Automatic. Ex Ord: Perturb Example Ordering.
}
\end{table*}

==> archived/tab_sensitivity_corr.tex <==
\begin{table*}[t]
\fontsize{9.5}{9.5}\selectfont
% \small
\setlength{\tabcolsep}{3pt}
\centering
\begin{tabular}{llccccccccccc}
\toprule
Adj. & Perturb & AG News & ARP & DBP & Emo & CARER & WikiQA & YAT & LYR & YRFS & MR & Avg \\
\cmidrule{2-13}
\multirow{3}{*}{None} & Inst - H & $\text{-0.438}^\dagger$ & $\text{-0.440}^\dagger$ & $\text{-0.203}^\dagger$ & $\text{-0.228}^\dagger$ & -0.156 & -0.113 & -0.149 & $\text{-0.424}^\dagger$ & $\text{-0.183}^\dagger$ & $\text{-0.328}^\dagger$ & -0.266 \\
\cmidrule{2-13}
& Inst - A & $\text{-0.272}^\dagger$ & $\text{-0.327}^\dagger$ & -0.167 & -0.089 & -0.111 & -0.302 & -0.192 & $\text{-0.343}^\dagger$ & $\text{-0.084}^\dagger$ & -0.157 & -0.204 \\
\cmidrule{2-13}
& Ex Ord & $\text{-0.145}^\dagger$ & $\text{-0.358}^\dagger$ & $\text{-0.159}^\dagger$ & $\text{\textbf{-0.295}}^\dagger$ & -0.080 & / & -0.132 & $\text{-0.590}^\dagger$ & $\text{-0.215}^\dagger$ & $\text{-0.322}^\dagger$ & -0.255 \\
\midrule
\multirow{3}{*}{CC} & Inst - H & $\text{\textbf{-0.501}}^\dagger$ & $\text{\textbf{-0.577}}^\dagger$ & $\text{-0.571}^\dagger$ & $\text{-0.097}^\dagger$ & $\text{\textbf{-0.359}}^\dagger$ & $\text{\textbf{-0.515}}^\dagger$ & $\text{-0.385}^\dagger$ & $\text{-0.472}^\dagger$ & $\text{-0.253}^\dagger$ & $\text{-0.336}^\dagger$ & -0.407 \\
\cmidrule{2-13}
& Inst - A & -0.228 & -0.269 & $\text{-0.382}^\dagger$ & $\text{0.000}$ & -0.136 & $\text{-0.391}^\dagger$ & $\text{-0.280}^\dagger$ & $\text{-0.328}^\dagger$ & $\text{-0.161}^\dagger$ & $\text{-0.370}^\dagger$ & -0.254 \\
\cmidrule{2-13}
& Ex Ord & $\text{-0.191}^\dagger$ & $\text{-0.484}^\dagger$ & $\text{-0.516}^\dagger$ & $\text{-0.282}^\dagger$ & $\text{-0.240}^\dagger$ & $\text{-0.310}^\dagger$ & $\text{-0.301}^\dagger$ & $\text{-0.567}^\dagger$ & $\text{-0.194}^\dagger$ & $\text{-0.419}^\dagger$ & -0.350 \\
\midrule
\multirow{3}{*}{PC} & Inst - H & $\text{-0.491}^\dagger$ & $\text{-0.541}^\dagger$ & $\text{-0.688}^\dagger$ & $\text{-0.274}^\dagger$ & $\text{-0.351}^\dagger$ & $\text{-0.065}^\dagger$ & $\text{-0.393}^\dagger$ & $\text{\textbf{-0.624}}^\dagger$ & $\text{-0.256}^\dagger$ & $\text{\textbf{-0.542}}^\dagger$ & \textbf{-0.422} \\
\cmidrule{2-13}
& Inst - A & $\text{-0.427}^\dagger$ & $\text{-0.445}^\dagger$ & $\text{-0.646}^\dagger$ & $\text{-0.269}^\dagger$ & $\text{-0.315}^\dagger$ & $\text{-0.185}^\dagger$ & $\text{\textbf{-0.540}}^\dagger$ & $\text{-0.507}^\dagger$ & $\text{-0.238}^\dagger$ & $\text{-0.337}^\dagger$ & -0.391 \\
\cmidrule{2-13}
& Ex Ord & $\text{-0.381}^\dagger$ & $\text{-0.459}^\dagger$ & $\text{\textbf{-0.822}}^\dagger$ & -0.159 & $\text{-0.333}^\dagger$ & -0.089 & $\text{-0.503}^\dagger$ & $\text{-0.518}^\dagger$ & $\text{\textbf{-0.258}}^\dagger$ & $\text{-0.471}^\dagger$ & -0.399 \\
\bottomrule
\end{tabular}
\caption{\label{tab:sensitivity-corr} The correlation between the sensitivity and accuracy of ICL predictions. We observe that sensitivity is negatively correlated with accuracy, with stronger correlation when decision boundary adjustment methods are applied to mitigate label bias. $^\dagger$ denotes correlations with $p$-value $< 0.05$. %Inst - H: human instruction perturbations. Inst - A: automatic instruction perturbations. Ex Ord: example ordering perturbations.
}
\end{table*}

==> tab_coverage_at_f1.tex <==
\begin{table*}[ht!]
\fontsize{9.5}{9.5}\selectfont
% \small
\setlength{\tabcolsep}{3pt}
\centering
\begin{tabular}{cccccccccc}
\toprule
& C@10 & C@20 & C@30 & C@40 & C@50 & C@60 & C@70 & C@80 & C@90 \\
\cmidrule{1-10}
AG News & 100 (100) & 100 (100) & 100 (100) & 100 (99) & 99 (96) & \textcolor{green!50!black}{93} (83) & 74 (62) & 19 (22) & 6 (4) \\
\cmidrule{1-10}
ARP & 100 (100) & 100 (100) & 100 (100) & 100 (100) & 100 (100) & 100 (99) & 99 (97) & 98 (96) & 97 (93) \\
\cmidrule{1-10}
DBP & 100 (100) & 100 (100) & 99 (98) & \textcolor{green!50!black}{91} (73) & \textcolor{green!50!black}{80} (49) & \textcolor{green!50!black}{66} (30) & \textcolor{green!50!black}{50} (16) & \textcolor{green!50!black}{35} (5) & \textcolor{green!50!black}{19} (1) \\
\cmidrule{1-10}
Emo & 100 (100) & \textcolor{green!50!black}{88} (78) & \textcolor{green!50!black}{64} (47) & \textcolor{green!50!black}{29} (11) & 7 (2) & 1 (0) & 1 (0) & 0 (0) & 0 (0) \\
\cmidrule{1-10}
CARER & 100 (100) & 100 (100) & \textcolor{green!50!black}{88} (74) & \textcolor{green!50!black}{46} (16) & \textcolor{green!50!black}{16} (3) & 1 (0) & 0 (0) & 0 (0) & 0 (0) \\
\cmidrule{1-10}
WikiQA & 100 (100) & 98 (94) & 84 (76) & \textcolor{green!50!black}{61} (50) & 9 (17) & 0 (1) & 0 (0) & 0 (0) & 0 (0) \\
\cmidrule{1-10}
YAT & 100 (100) & 100 (100) & 100 (99) & 81 (74) & \textcolor{green!50!black}{35} (25) & 4 (4) & 1 (0) & 0 (0) & 0 (0) \\
\cmidrule{1-10}
LYR & 100 (100) & 100 (100) & 100 (100) & 100 (100) & 100 (100) & 100 (100) & 100 (100) & 100 (100) & \textcolor{green!50!black}{95} (74) \\
\cmidrule{1-10}
YRFS & 100 (100) & 100 (100) & 100 (100) & 95 (88) & \textcolor{green!50!black}{45} (34) & 4 (2) & 1 (0) & 0 (0) & 0 (0) \\
\cmidrule{1-10}
MR & 100 (100) & 100 (100) & 100 (100) & 100 (100) & 100 (100) & 100 (100) & 100 (100) & 99 (98) & \textcolor{green!50!black}{89} (71) \\
\bottomrule
\end{tabular}
\caption{\label{tab:cov_at_f1} We report the Coverage@F1 scores for our \textsc{SelSen} method under the prototypical calibration setting, and compare to the \textsc{MaxProb} baseline (scores shown in parentheses). C@X: coverage rate at F1 score X. Our method consistently gets higher Coverage@F1 scores compared to the \textsc{MaxProb} baseline on all ten tasks across different F1 thresholds. We color the scores \textcolor{green!50!black}{green} if our \textsc{SenSel} method outperforms the \textsc{MaxProb} baseline by at least 10 coverage points.}
\end{table*}
